On the Optimization Landscape of Tensor Decompositions

Non-convex optimization with local search heuristics has been widely used in machine learning, achieving many state-of-art results. It becomes increasingly important to understand why they can work for these NP-hard problems on typical data. The landscape of many objective functions in learning has been conjectured to have the geometric property that "all local optima are (approximately) global optima", and thus they can be solved efficiently by local search algorithms. However, establishing such property can be very difficult. In this paper, we analyze the optimization landscape of the random over-complete tensor decomposition problem, which has many applications in unsupervised learning, especially in learning latent variable models. In practice, it can be efficiently solved by gradient ascent on a non-convex objective. We show that for any small constant $\epsilon > 0$, among the set of points with function values $(1+\epsilon)$-factor larger than the expectation of the function, all the local maxima are approximate global maxima. Previously, the best-known result only characterizes the geometry in small neighborhoods around the true components. Our result implies that even with an initialization that is barely better than the random guess, the gradient ascent algorithm is guaranteed to solve this problem. Our main technique uses Kac-Rice formula and random matrix theory. To our best knowledge, this is the first time when Kac-Rice formula is successfully applied to counting the number of local minima of a highly-structured random polynomial with dependent coefficients.

==> aug_stripped.tex <==







==> basics_stripped.tex <==




==> estimation.tex <==


\section{Bounding the number of local minima using Kac-Rice Formula}\label{sec:global}
%In this section we prove Theorem~\ref{thm:kac-rice-zero} using Kac-Rice Formula. 
%
%
%Let $E_0$ be the event that 





%\FIXME{Define $\tau = Kn/d$. }
%\begin{theorem}
%	\begin{align}
% \Exp\left[\Exp\left[\left|\det(M)\right|\indicator{M\succeq 0} \indicator{E_0}\indicator{E_1}\mid g = 0,\alpha\right] p_{g\mid \alpha}(0)\right] \ll 1
%	\end{align}	
%\end{theorem}
%Define
%\begin{align}
%	W(\alpha) & = \Exp\left[\det(M)\indicator{M\succeq 0}\indicator{E_1}\mid g = 0, \alpha\right] \indicator{E_0}  \
%\end{align}



In this section we give the proof of Proposition~\ref{prop:f_0} and Proposition~\ref{prop:f_k}, using the intuition described in Section~\ref{sec:proof_sketches}. 
\subsection{Proof of Proposition~\ref{prop:f_0}}

%
%For the ease of exposition, define $W(\alpha)$ as 
%\begin{align}
%W(\alpha) = \Exp\left[\det(M)\indicator{M\succeq 0}\indicator{E_2'}\mid g = 0, \alpha\right]\indicator{E_0}\indicator{E_1}\indicator{E_2}   \label{eqn:def-Walpha}
%\end{align}
%
%Therefore we have that 
%\begin{align}
%h(\alpha) = \Vol(\sphere^{d-1})  W(\alpha)  p_{g\mid \alpha}(0)\label{def:Wa}\end{align}
%
%
%Towards estimating $\Exp\left[h(\alpha)\indicator{F_0}\right]$, we fix a choice of $\alpha$ and start to $W(\alpha)\indicator{F_0}$ first. Here an apparent difficulty is to handle the determinate $\det(M)$. Fortunately we have the following simple claim that bounds the determinate from above by the trace. 
%\begin{claim}\label{claim:amgm}
%	For any $p\times p$ symmetric matrix $V$, we have, 
%\begin{align}
%		\det(V)\indicator{V\succeq 0}& \le \left(\frac{|\trace(V)|}{p}\right)^p\indicator{V\succeq 0} \nonumber
%\end{align}
%\end{claim}
%The claim is a direct consequence of AM-GM inequality. 
%\begin{proof}
%	We can assume $V$ is positive semidefinite since otherwise both sides of the inequality vanish. Then, suppose $\lambda_1,\dots, \lambda_p \ge 0$ are the eigenvalues of $V$. We have $\det(V) = \lambda_1\dots \lambda_p$ and $|\trace(V)| = \trace(V) = \lambda_1+\dots +\lambda_p$. Then by AM-GM inequality we complete the proof. 
%\end{proof}
%Applying Claim~\ref{claim:amgm} with $V = M$, we have the following direct corollary, 
Following the plan in Section~\ref{sec:proof_sketches}, we start with using AM-GM inequality for the determinant. 
\begin{lemma}\label{cor:det-to-trace-app}
	Under the setting of Proposition~\ref{prop:f_0}, we have, 
	\begin{align}
		W(\alpha)\indicator{F_0} \Ezero\Etwo\Etwo\le \Exp\left[\frac{|\trace(M)|^{d-1}}{(d-1)^{d-1}} \mid g = 0, \alpha\right] \indicator{F_0}\indicator{E_0} \Eone\Etwo \nonumber\mper
	\end{align}
\end{lemma}

The next thing that we need to bound is $\Exp\left[|\trace(M)|^{d-1} \mid g, \alpha\right]$. Here the basic intuition is that since $\trace(M)\mid g,\alpha$ is quite concentrated around its mean and therefore we can switch the $(d-1)$-th power with the expectation without losing much. Proving such a result would require the understanding of the distribution of $M\mid g,\alpha$. We have the following  generic Claim that computes this distribution in a more general setting. 

\begin{claim}\label{claim:remove_conditioning}
	Let $w,y\in \R^n$ be two fixed vectors, and let $\bar{q} = y^{\odot 3}/\norm{ y^{\odot 3}}$. 
	Let $B = [b_1,\dots, b_n]\in \R^{(d-1)\times n}$ be a matrix with independent standard Gaussians as entries. Let $M_w = \|w\|_4^4\cdot\Id_{d-1} -3\sum_{i=1}^{n}w_i^2 b_ib_i^{\top}$ and $g_y  = \sum_{i=1}^{n}y_i^3 b_i$. 
	Let $Z\in \R^{(d-1)\times n}$ be a random matrix with rows independent drawn from $\N(0,\Id_n - \bar{q}\bar{q}^{\top})$. 
	
	Then, we have that $B \mid (g_y = 0)$ has the same distribution as $Z$, and consequently $M_w\mid g_y = 0$ has the same distribution as 
	\begin{align}
\fourmoments{w}\Id_{d-1} - 3Z\diag(w^{\odot 2})Z^{\top}\mper\nonumber
	\end{align}
\end{claim}

One can see that the setting that we are mostly interested in corresponds to $w = y=\alpha$ in Claim~\ref{claim:remove_conditioning}. 
\begin{proof}
	%Let $q = (y_1^3,\dots, y_n^3)^{\top}\in \R^n$, and let $\bar{q} = q/\|q\|$. 
	%Let $B = [b_1,\dots, b_n]\in \R^{(d-1)\times n}$ and 
	Let $c_1^{\top},\dots, c_{d-1}^{\top}$ be the rows of $B$. We write $c_i =\beta_i\bar{q} + z_i$ where $\beta_i = \inner{c_i,\bar{q}}$ and $z_i = (\Id_n-\bar{q}\bar{q}^{\top})c_i$. Let $Z$ denote the matrix with $z_i^{\top}$ as rows. Therefore we have $B = Z + \beta \bar{q}^{\top}$. %and let $\hat{b}_j$ be its $j$-th columns. %Therefore in this notation, $b_j = \hat{b}_j + $
	
	Recall that $b_i$ are independent Gaussians with covariance $\N(0,\Id_{d-1})$. Thus we have that $c_i$'s are independent Gaussians with covariance $\N(0,\Id_n)$, and consequently $\beta_i$ and $z_i$ are independent random variables with $\N(0, 1)$ and $\N(0,\Id_n - \bar{q}\bar{q}^{\top})$ respectively. Moreover, note that $g = 0$ is equivalent to that $\forall i\in [d-1], \inner{c_i,q} = 0$, which in turn is equivalent to that $\forall i\in [d-1], \beta_i = 0$. Hence, $B \mid (g_y = 0)$ has the same distribution as $Z$, and consequently $M_w\mid (g_y=0)$ has the same distribution as $\|w\|_4^4\Id_{d-1} - 3Z\diag(w^{\odot 2})Z^{\top}$. 
\end{proof}

Using Claim~\ref{claim:remove_conditioning}, we can compute the the expectation of the trace and its $p$-th moments. Again we state the following proposition in a more general setting for future re-usability. 
\begin{proposition}\label{prop:det-to-trace}
	In the setting of Claim~\ref{claim:remove_conditioning}, we have
	\begin{align}
	\Exp\left[\trace(M_w)\mid g_y\right] = (d-1)\left(\|w\|_4^4 - 3\|w\|^2 + 3\inner{y^{\odot 6},w^{\odot 2}}/\|y\|_6^6\right)\mper \nonumber
	\end{align}
	Moreover,  for any $\epsilon \in (0,1)$, 
	\begin{align}
	\Exp\left[|\trace(M_w)|^p\mid g_y = 0\right]\le \max\left\{(1+\epsilon)^p \left|\Exp\left[\trace(M_w)\mid g_y\right]\right|^p, (\frac{1}{\epsilon}+1)^p\max\{4p\|w\|_{\infty}^2, 2 \sqrt{pd}\|w\|_4^2\}^p\right\} \label{eqn:21}
	\end{align}
\end{proposition}

\begin{proof}[Proof of Proposition~\ref{prop:det-to-trace}]
We use the same notations as in the proof of Claim~\ref{claim:remove_conditioning}.	
By Claim~\ref{claim:remove_conditioning}, we have $B =[b_1,\dots, b_n] \mid (g_y = 0)$ has the same distribution as $Z$, and consequently $M_w\mid (g_y=0)$ has the same distribution as $\|w\|_4^4\Id_{d-1} - 3Z\diag(w^{\odot 2})Z^{\top}$. 
	Furthermore, this implies that $\trace(M_w \mid (g_y = 0))$ has the same distribution as the random variable (denoted by $\Gamma$ below)
	\begin{align}
	\Gamma := \trace\left(\|w\|^4\Id_{d-1} - 3Z\diag(w^{\odot 2})Z^{\top}\right) = (d-1)\|w\|_4^4 - 3\sum_{k\in [d-1]} \|z_k\odot w\|^2\mper
	\end{align}
	
	
Since $z_k\odot w$ is Gaussian random variable, we have that $\|z_k\odot w\|^2$ is a sub-exponential random variable with parameter $(\nu,\rho)$ satisfying  $\nu\lesssim \|w\|_4^2$ and $\rho\lesssim \|w\|_{\infty}^2$ (see Definition~\ref{def:sub-exponential} for the definition of sub-exponential random variable and see Lemma~\ref{lem:zwnorm} for the exact calculation of the parameters for this case) . It is well known that when one takes sum of independent sub-exponential random variable, the $\rho$ parameter will be preserved and $\nu^2$ (which should be thought of as variance) will added up (see Lemma~\ref{lem:sub-exp-addition} for details).   Therefore, we have that $\Gamma$ is a sub-exponential random variable with parameter $(\nu^*, \rho^*)$ satisfying $\nu^* \lesssim \sqrt{d-1}\|w\|_4^2$ and $\rho^*\lesssim \|w\|_{\infty}^2$. Moreover, by Lemma~\ref{lem:zwnorm} again and the linearity of expectation,  we can compute the expectation of $\Gamma$,  \begin{align}
	\Exp\left[\Gamma\right] = (d-1)\left(\|w\|_4^4 - 3\|w\|^2 + 3\inner{\bar{q}^{\odot 2},w^{\odot 2}}\right) \mper\label{eqn:8} 
	\end{align} 
Next the basic intuition is if $\nu^*$ and $\rho^*$ are small enough compared to the mean of $\Gamma$, then $\Gamma$ is extremely concentrated around its mean, and thus $\Exp\left[|\Gamma|^{p} \right]$ is close to $\Exp\left[\Gamma\right]^p$. Otherwise, the mean is more or less negligible compared to $\max\{p\norm{w}_{\infty}, 2\sqrt{pd}\norm{w}_4^2\}$,  then  the moment of $\Gamma$ behaves like the moments of an sub-exponential random variable with mean 0. 	Indeed, using basic integration, we can show (see Lemma~\ref{lem:sub-exp-before_truncation-moments}) that a sub-exponential random variable with mean $\mu$ and parameter $(\nu,b)$ satisfies that for any $\epsilon\in (0,1)$, 
\begin{align}
		\Exp |X|^p  \lesssim \frac{1}{\epsilon^{p-1}} |\mu|^p + \frac{1}{(1-\epsilon)^{p-1}} \left(\nu^p p!! + (2b)^p p!\right)\mper \nonumber
		\end{align}
		Applying the equation above to $\Gamma$ completes the proof. 
\end{proof}

Using Proposition~\ref{prop:det-to-trace} with $w = y=\alpha$. we obtain the following bounds for the moments of the trace of $M$. 

\begin{corollary}\label{cor:tracepower} For any fixed $\alpha$, we have
		\begin{align}
		\Exp\left[\left(\frac{|\trace(M)|}{d-1}\right)^{p}\mid g = 0, \alpha\right] \indicator{E_0}\indicator{E_2}
		& \lesssim (1+O(\delta))^{p} \max\left\{Q(\alpha)^p, (0.1d)^p, \left(0.1pd^{-1/2}n^{1/2}\right)^{p}\right\}\mper\nonumber
		\end{align}
\end{corollary}

\begin{proof}
	We fix the choice of $\alpha$ and assume it satisfies event $F_0$. We will apply Proposition~\ref{prop:det-to-trace} with $w = \alpha$ and $y = \alpha$. We can verify that when $E_0$ and $E_2$ both happen, we have
	\begin{align}
	\max\{4p\|w\|_{\infty}^2, 2\sqrt{pd}\norm{w}_4^2\} & \lesssim  \max\{p\|\alpha\|_{\infty}^2, p\norm{\alpha}_4^2\} \le p\norm{\alpha}_{\infty}\Norm{\alpha}_2\nonumber \\
	& \lesssim \delta pd^{1/2}n^{1/2}\mper\tag{since $\alpha$ satisfies event $E_0,E_2$}
	\end{align}
	Therefore, taking $\epsilon = O(\delta)$ in Proposition~\ref{prop:det-to-trace}, we have that 
	\begin{align}
	\Exp\left[|\trace(M)|^{p}\mid g = 0, \alpha\right] \indicator{E_0}\indicator{E_2}\lesssim (1+O(\delta))^{p} \max\left\{\mu^{p}, \left(0.1pd^{1/2}n^{1/2}\right)^{p}\right\} \nonumber\mcom
	\end{align}
	where $\mu = \left|\Exp\left[\trace(M)\right]\right| = (d-1) (\|\alpha\|^4 - 3\|\alpha\|^2 + \frac{3\|\alpha\|_8^8}{\|\alpha\|_6^6})$. When $E_0$ happens, we have $\mu \le (d-1)(\Norm{\alpha}_4^4-3\Norm{\alpha}^2 + 3\Norm{\alpha}_{\infty}^2) \le (d-1)(\Norm{\alpha}_4^4-3\Norm{\alpha}^2 + O(\delta d))$. It follows that 
	\begin{align}
	\Exp\left[\left(\frac{|\trace(M)|}{d-1}\right)^{p}\mid g = 0, \alpha\right] \indicator{E_0}\indicator{E_2}& \lesssim (1+O(\delta))^{p} \max\left\{(Q(\alpha) + O(\delta d))^p, \left(0.1pd^{-1/2}n^{1/2}\right)^{p}\right\}\mper\nonumber\\
& \lesssim (1+O(\delta))^{p} \max\left\{Q(\alpha)^p, (0.1d)^p, \left(0.1pd^{-1/2}n^{1/2}\right)^{p}\right\}\mper %\tag{\FIXME{maybe add explanation}}
	\end{align}
\end{proof}

Putting Corollary~\ref{cor:tracepower} and Lemma~\ref{cor:det-to-trace-app} together, we can prove Proposition~\ref{prop:f_0}. 
\begin{proof}[Proof of Proposition~\ref{prop:f_0}]

	Moreover, when $E_0$ happens, we have, 
	\begin{align}
	p_{g\mid \alpha}(0) &= (2\pi)^{-d/2} (\Norm{\alpha}_6^6)^{-d/2} \label{eqn:41}\\
	& \le (1+O(\delta))^d (2\pi)^{-d/2} (15n)^{-d/2}\label{eqn:44}\mper
	\end{align}
	It follows that 
	\begin{align}
	%\Exp\left[h(\alpha)\indicator{F_0}\right] & = 
	\Exp\left[  W(\alpha)  p_{g\mid \alpha}(0)\right] &	\le (1+O(\delta))^d (30\pi n)^{-d/2} \Exp\left[\Exp\left[\left|\frac{\trace(M)}{d-1}\right|^{(d-1)}\mid g = 0, \alpha\right] \indicator{E_1}\indicator{E_2}\indicator{F_0}\right] \tag{by Corollary~\ref{cor:det-to-trace-app}}\\
	&\le (1+O(\delta))^d (30\pi n)^{-d/2}\Exp\left[\max\left\{Q(\alpha)^{d-1}, (0.1d)^{d-1}, \left(0.1d^{1/2}n^{1/2}\right)^{p}\right\}\indicator{E_1}\indicator{F_0}\right]\tag{by Corollary~\ref{cor:tracepower} with $p = d-1$}\\
	&\le (1+O(\delta))^d (30\pi n)^{-d/2}\Exp\left[\max\left\{Q(\alpha_S)^{d-1},  \left(0.1d^{1/2}n^{1/2}\right)^{p}\right\}\indicator{E_1}\right] \label{eqn:11}
	%& \le (1+O(\delta))^d (30\pi n)^{-d/2}\Exp\left[(\sum_{i\in [n]}(\alpha_i^4-3\alpha_i^2)\indicator{|\alpha_i|\le \tau^{1/4}})^d\indicator{E_1}\right] \nonumber\\
	%& ~~+ (1+O(\delta))^d (30\pi n)^{-d/2}d^d\tag{\FIXME}
	\end{align}
	%\FIXME{informal argument below}
	%Observe that $\left(\|\alpha\|^4 - 3\|\alpha\|^2 \right)\indicator{F_0} \le \left(\sum_{i\in [n]}(\alpha_i^4-3\alpha_i^2)\indicator{|\alpha_i|\le \tau^{1/4}}\right)$. 
	For simplicity, Let $Z_i = (\alpha_i^4-3\alpha_i^2)\indicator{|\alpha_i|\le \tau^{1/4}}$, and $Z = \sum_i Z_i$. We observe that $E_1$ and $E_0$ implies that $Z\ge (\gamma-3)\sqrt{nd}$. Let $\gamma'=\gamma-3$.
	Thus, $Z^d\indicator{Z\ge {\gamma'} \sqrt{nd}}\le (\sum_{i\in [n]}(\alpha_i^4-3\alpha_i^2)\indicator{|\alpha_i|\le \tau^{1/4}})^d\indicator{E_1}$.  Then, 
%	
%	\begin{align}
%	\Exp\left[  W(\alpha)  p_{g\mid \alpha}(0)\right] 
%	& \le (1+O(\delta))^d (30\pi n)^{-d/2}\Exp\left[|Z|^d\indicator{Z\ge {\gamma'} \sqrt{nd}}\right]  + (1+O(\delta))^d (30\pi n)^{-d/2}d^d\label{eqn:42}\mper
%	\end{align}
	\begin{align}
	\Exp\left[Q(\alpha_S)^{d-1}\Eone\right] = \Exp\left[|Z|^{d-1}\indicator{Z\ge {\gamma'}\sqrt{nd}}\right]\label{eqn:15}
	\end{align}
We have that $Z_i$ is a sub-exponential variable with parameter $(\sqrt{41}, (4+o_{\tau}(1))\tau^{1/2})$ (by Lemma~\ref{lem:bernstein_moment}). Then by Lemma~\ref{lem:sub-exp-addition}, we have that $\sum_i Z_i$ is sub-exponential with parameters $(\sqrt{41n}, (4+o_{\tau}(1))\tau^{1/2})$. Moreover, we have $Z$ has mean $o_d(n)$ since $n \ge d\log d$. 
	
	Then, we use Lemma~\ref{lem:sub_exponential_moments} to control the moments the sub-exponential random variable $Z\cdot \indicator{|Z|\ge {\gamma'} \sqrt{nd}}$. Taking $s = {\gamma'} \sqrt{nd}$ and $\nu = \sqrt{41n}$ and $b= (4+o_{\tau}(1))\tau^{1/2}$ in Lemma~\ref{lem:sub_exponential_moments}, we obtain that when when ${\gamma'} \ge \max\{\sqrt{41}, (1+\eta)(8+o_{\tau}(1))\sqrt{\tau d/n}\} = \max\{\sqrt{41}, (1+\eta)(8+o_{\tau}(1))\sqrt{K}\}$
	\begin{align}
		\Exp\left[|Z|^{d-1} \indicator{Z\ge {\gamma'} \sqrt{nd}}\right]\le o_d(n)/\epsilon^{d} + \frac{1}{(1-\epsilon)^d}\left((1+o(1))^dd^2e^{-{\gamma'}^2d/82} +1/\eta \cdot e^{-(1/8-o_{\tau}(1)){\gamma'}/\sqrt{K}}\right)\nonumber\mper
	\end{align}
	Take $\epsilon = 1/\log d$ and $\eta = 1/\log d$,  we obtain that 
	\begin{align}
	\Exp\left[|Z|^{d-1} \indicator{Z\ge {\gamma'} \sqrt{nd}}\right]\le (1+o(1))^d ({\gamma'} \sqrt{nd})^{d/2}\left(e^{-{\gamma'}^2d/82} + \cdot e^{-(1/8-o_{\tau}(1)){\gamma'}/\sqrt{K}}\right)\label{eqn:38}\mper
	\end{align}
Hence, combing equation~\eqref{eqn:11}, ~\eqref{eqn:15} and~\eqref{eqn:38}, we have, %recalling that $\tau = K n/d$, we have, 
	\begin{align}
			\Exp\left[h(\alpha)\indicator{F_0}\right] & \lesssim  \Vol(\sphere^{d-1}) \Exp\left[W(\alpha)  p_{g\mid \alpha}(0)\right]\tag{by equation~\eqref{def:Wa}} \\
			&\lesssim \frac{\pi^{d/2}}{(d/(2e))^{d/2}} \cdot (1+o(1))^d (30\pi n)^{-d/2}({\gamma'}^2 nd)^{d/2}\left(e^{-{\gamma'}^2d/82} + \cdot e^{-(1/8-o_{\tau}(1)){\gamma'}/\sqrt{K}}\right) \nonumber\\
			& \lesssim(1+o(1))^d \left(\frac{e{\gamma'}^2}{15}\right)^{d/2}\left(e^{-{\gamma'}^2d/82} + \cdot e^{-(1/8-o_{\tau}(1)){\gamma'}/\sqrt{K}}\right)\le 2^{-d/2}\mper \tag{Since ${\gamma'}$ is a sufficiently large constant that depends on the choice of $K$}
	\end{align}
\end{proof}


\subsection{Proof of Proposition~\ref{prop:f_k}}

%Let $Q(\cdot): \R^d \rightarrow \R$ defined as: 
%\begin{align}
%Q(z) = \Norm{z}_4^4 - 3\Norm{z}^2 \label{eqn:def:Q}\mper
%\end{align}

In the proof of Proposition~\ref{prop:f_k}, we will have another division of the the coordinates of $\alpha$ into two subsets $S$ and $L$ according to the magnitude of $\alpha_i$'s. Throughout this subsection, let $C$ be a sufficiently large constant that depends on $\delta$. Let $S = \{i: |\alpha_i| \le \sqrt{C\log d}\}$ and $L = [n]\backslash S$. Thus by definition, since $n \ge d\log^2 d$, we have that event $F_k$ implies that $k\in L$. But we note the threshold $\sqrt{C\log d}$ here is smaller than the threshold $\tau = Kn/d$ for defining event $F_k$'s. The key property that we use here is that the set $L$ have cardinality at most $d$ as long as $E_0$ happens. This will allows us to bound the contribution of the coordinates in $L$ in a more informative way.

\begin{claim}\label{claim:sizeL}
	Let $S,L$ are defined as above with $C\ge 2/\delta$. Suppose $E_0$ happens, then we have $|L|\le \delta n/\log d$. 
\end{claim}
\begin{proof}
	Assume for the sake of contradiction that $|L| > \delta n/\log d$, then we can pick a subset $L'\subset L$ of size $\delta n/\log d$ and obtain that $\norm{\alpha_{L'}}^2 \ge |L'| C\log d= \delta d C \ge 2d$ which violates~\eqref{eqn:RIP}.
\end{proof}

For notational convenience, let $P = (2-O(\delta))\tau^{1/2}d = (2-O(\delta))\sqrt{Knd}$. Recall $\alpha_S$ is the restriction of vector $\alpha$ to the coordinate set $S$, and $Q(\cdot): \R^d \rightarrow \R$ is defined as: 
\begin{align}
Q(z) = \Norm{z}_4^4 - 3\Norm{z}^2 \nonumber\mper
\end{align}
Define $T_1(\alpha),T_2(\alpha)$ as\begin{align}
T_{1}(\alpha) & =  \exp\left(-\frac{(P-Q(\alpha_S))^2}{36\norm{\alpha_S}_4^4}\right)\nonumber\\
T_{2}(\alpha) &=  \indicator{P \le Q(\alpha_S)}\mper\label{eqn:def-T12}
\end{align}

Therefore, since $Q(\alpha_S) = \norm{\alpha_S}_4^4-3\norm{\alpha_S}^2$ is roughly a random variable with standard deviation $\Theta(\sqrt{n})$, for large enough constant $K$, we should think of $T_1(\alpha)$ and $T_2(\alpha)$ as exponentially small random variable.  The following Lemma is the key of this section, which says that when $F_0$ happens, the chance of $M$ being PSD is very small. 

\begin{lemma}\label{lem:prob_indicator} In the setting of Proposition~\ref{prop:f_k}, let $T_{1}(\alpha),T_2(\alpha)$ be defined as in~\eqref{eqn:def-T12}. Then,
	\begin{align}
	\Exp\left[\indicator{M\succeq 0} \indicator{E_2'}\mid g, \alpha \right] \indicator{F_k} \indicator{E_0}\le T_{1}(\alpha) + T_2(\alpha) \mper\nonumber
	\end{align}
	\Tnote{We might be able to get slightly smaller constant}
\end{lemma}

\begin{proof}\Tnote{This proof requires another round of proofread}
	We assume throughout this proof that $\alpha$ is a fixed vector and that $\alpha$ satisfies $F_k$ and $E_0$. %Thus, we omit the indicator $\indicator{F_k}$ and $\indicator{E_0}$ in the proof. 
	For simplicity, define $\hat{\tau} = \sqrt{C\log d}$. 
	
	Let $q = (\alpha_1^3,\dots, \alpha_n^3)^{\top}\in \R^n$, and $\bar{q} = q/\|q\|$.	Let $z_1,\dots z_{d-1}$ be i.i.d Gaussian random variables in $\R^d$ with covriance $\N(0,\Id_n-\bar{q}\bar{q}^{\top})$. Let $Z$ denote the matrix with $z_i^{\top}$ as rows and let $v_j~(j\in [n])$ denotes the $j$-th column of $Z$. Then, by Claim~\ref{claim:remove_conditioning}, random variable $(M, \indicator{E_2'})\mid g = 0, \alpha)$ has the same joint distribution as $(M', \indicator{E_2''})$ defined below \Tnote{To add explanation},
	\begin{align}
	M' = \|\alpha\|_4^4\cdot \Id_{d-1} -3\sum_{i\in [n]} \alpha_i^2v_iv_i^{\top}, E_2'' = \Set{\forall i, \|v_i\|^2 \ge (1-\delta)d} \mper\nonumber
	\end{align}
	Then, it suffices to bound from above the quantity 	$	\Pr\left[M'\succeq 0\wedge E_2''\right]\mper$
	
	A technical complication here is that $v_1,\dots, v_n$ are not independent random variables. We get around this issue by the following ``coupling'' technique which introduces some additional randomness. Let $\beta\in \N(0,\Id_{d-1})$ be a random variable that is independent with all the $v_i$'s and  define $\tilde{B} = \beta\bar{q}^{\top}  + Z$. We can verify that $\tilde{B}$ contains independent entries with distribution $\N(0,1)$. Let $\tilde{b}_1,\dots, \tilde{b}_n$ be the columns of $\tilde{B}$. Let $\bar{v}_k = v_k/\norm{v_k}$.  We have that $M'\succeq 0$ implies that 
	\begin{align}
	\bar{v}_k^{\top}M'\bar{v}_k= \|\alpha\|_4^4 - 3\sum_{i\in [n]}\alpha_i^2 \inner{v_i,\bar{v}_i}^2 \ge 0 \mper\label{eqn:23}
	\end{align}
	We bound from above $\bar{v}_k^{\top}M'\bar{v}_k$ by decomposing it according to the subset $S,L$. 
	\begin{align}
	\bar{v}_k^{\top}M'\bar{v}_k & = \norm{\alpha_{S}}_4^4 -3 \sum_{i\in S}\alpha_i^2 \inner{v_i,\bar{v}_i}^2 + \norm{\alpha_L}_4^4 - 3\sum_{i\in L} \alpha_i^2 \inner{v_i,\bar{v}_i}^2 \nonumber\\
	&\le \underbrace{\norm{\alpha_{S}}_4^4 - 3\sum_{i\in S}\alpha_i^2 \inner{v_i,\bar{v}_i}^2}_{A_S} + \underbrace{\norm{\alpha_L}_4^4 - 3\alpha_k^2\inner{v_k,\bar{v}_k}^2}_{A_L} \label{eqn:24}
	\end{align}
	Here $A_S, A_L$ are defined above in equation~\eqref{eqn:24}. 
	By Claim~\ref{claim:sizeL}, we have $|L| \le \delta n/\log d$.  By~\eqref{eqn:RIP} again, we have that $E_0$ implies that $\norm{\alpha_L}^2\le (1+\delta)d$. 
	%we have that $(1+\delta) n\ge\norm{\alpha}^2\ge  \norm{\alpha_L}^2\ge C|L|$, and it follows that $|L|\le (1+\delta)n/C$.Thus for sufficiently large constant $C$, we have $|L|\le \delta n$ and by equation~\eqref{eqn:RIP}, we have that $E_0$ implies that $\norm{\alpha_L}^2 \le (1+\delta)n$. 
	Then, we have $\norm{\alpha_L}_4^4 \le \max_i \alpha_i^2 \cdot \norm{\alpha_L}^2\le (1+\delta)d\max_i \alpha_i^2 = (1+\delta)d\alpha_k^2$. Moreover, when $E_2''$ happens, we have that $\alpha_k^2\inner{v_k,\bar{v}_k}^2 = \alpha_k^2\norm{\bar{v}_k}^2 \ge \alpha_k^2 (1-\delta)d $. Thus, %Therefore, $\bar{G}_1$ and $E_1$ implies that 
	\begin{align}
	A_L\cdot \indicator{E_2''} &= (\norm{\alpha_L}_4^4 - 3\alpha_k^2\inner{v_k,\bar{v}_k}^2)\indicator{E_2''}  \le (1+\delta)d\alpha_k^2 - 3\alpha_k^2(1-\delta)d \nonumber\\ & \le - (2-O(\delta))\alpha_k^2 d \le -(2-O(\delta))\sqrt{\tau}d\label{eqn:25}
	\end{align}
	Then combining equation~\eqref{eqn:23}, ~\eqref{eqn:24} and~\eqref{eqn:25},  we have that when $M'\succeq 0$ and $E_2''$ both happen, it holds that $A_S\ge (2-O(d))\tau^{1/2}d$. 
	
	\Tnote{Require edits below}
	
	Next we consider in more detail the random variable $A_S$. Define random variable $Y = \bar{v}_k^{\top} \tilde{B}_{-k}\diag((\alpha_{S})_{-k})$, where $\tilde{B}_{-k}$ is the $(d-1)\times (n-1)$ sub-matrix of $\tilde{B}$ that excludes the $k$-th column of $\tilde{B}$, and $(\alpha_{S})_{-k}$ is the $n-1$-dimensional vector that is obtained from removing the $k$-th entry of $\alpha_S$. Note that since $k\not\in S$, we have that $\norm{Y}^2 = \sum_{i\in S}\alpha_i^2 \inner{v_i,\bar{v}_i}^2$, and $A_S  = \norm{\alpha_S}_4^4 - 3\norm{Y}^2$. Thus our goal next is to understand the distribution of $Y$. 
	
	We observe that $Y\mid v_k$ is a Gaussian random variable since $\tilde{B}_k\mid v_k$ is a Gaussian random variable. Let $\ell_i\in \R^{n-1}$ denote the $i$-th row of the matrix $\tilde{B}$. Then $\ell_1,\dots, \ell_{d-1}$ are i.i.d Gaussian random variable with distribution $\N(0,\Id_{n})$. Now we consider $\ell_i\mid v_{k,i}$, where $v_{k,i}$ is the $i$-th coordinates of vector $v_k$.  Note that $v_{k,i} = z_{i,k} = ((\Id-\bar{q}\bar{q}^{\top})\ell_i)_k = \inner{e_k- \bar{q}_k\bar{q}, \ell_i}$ (here $z_{i,k}$ denotes the $k$-th coordinate of $z_i$ and $e_k$ is the $k$-th natural basis vector in $\R^n$). Thus, conditioning on $v_{k,i}$ imposes linear constraints on $\ell_i$. Let $s_k = e_k- \bar{q}_k\bar{q}\in \R^n$ and $\bar{s}_k  = s_k/\norm{s_k}$. Then $\ell_i \mid v_{k,i}$ has covariance $\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}$. %Denote by $\mu_k$.
	Computing the mean of $\ell_i \mid v_{k,i}$  will be tedious but fortunately our bound will not be sensitive to it. Now we consider random variable  $\ell_i' = (\ell_i)_{-k}\diag((\alpha_{S})_{-k})\mid v_{k,i}$ in $\R^{n-1}$ where $(\ell_i)_{-k}$ denotes the restriction of $\ell_{i}$ to the subset $[n]\backslash \{k\}$. Note that $\ell_i'$ is precisely a row of  $\tilde{B}_{-k}\diag((\alpha_{S})_{-k})$. We have $\ell_i'$ is again a Gaussian random variable and its covariance matrix is $\Sigma = \diag((\alpha_{S})_{-k})\left(\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}\right)_{-k,-k}\diag((\alpha_{S})_{-k})$, where $\left(\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}\right)_{-k,-k}$ is the restriction of $\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}$ to the subsets $([n]\backslash \{k\})\times ([n]\backslash \{k\})$. Since $\ell_i$'s are independent with each other, we have $Y^{\top} \mid \bar{v}_k= [\ell_1',\dots, \ell_{d-1}']\cdot \bar{v}_k$  is Gaussian random variable with covariance $\|\bar{v}_k\|^2\Sigma = \Sigma$. 
	
	Next we apply Lemma~\ref{lem:norm_concentration} on random variable $Y^{\top}$ and obtain that $Y^{\top}$ has concentrated norm in the sense that for any choice of $v_k$, 
	\begin{align}
	\Pr\left[\norm{Y}^2 \ge \trace(\Sigma) -\norm{\Sigma} - 2\sqrt{\trace(\Sigma^2)t}\mid v_k\right]\ge 1-e^{-t} \mper\label{eqn:30}
	\end{align}
	
	Recall that $\Sigma = \diag((\alpha_{S})_{-k})\left(\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}\right)_{-k,-k}\diag((\alpha_{S})_{-k})$. Therefore, we have $\trace(\Sigma) = \sum_{i\in S}\alpha_i^2 - \norm{\bar{s}_k\odot (\alpha_S)_{-k}}^2\ge \sum_{i\in S}\alpha_i^2 - \norm{\alpha_S}_{\infty}^2\ge \sum_{i\in S}\alpha_i^2 - \hat{\tau}^{1/2}$. Moreover, we have that $\norm{\Sigma}\le \norm{\alpha_S}^2\le \hat{\tau}^{1/2}$ and $\trace(\Sigma^2)\le \norm{\alpha_S}_4^4$.  Plugging these into equation~\eqref{eqn:30}, and using the fact that $A_S  = \norm{\alpha_S}_4^4 - 3\norm{Y}^2$, we have that for any $t\ge 0$, 
	\begin{align}
	\Pr\left[A_S \ge \norm{\alpha_S}_4^4 - 3 \norm{\alpha_S}^2 + 6\hat{\tau}^{1/2} + 6\sqrt{\norm{\alpha_S}^4_4 t}\mid v_k\right]\le e^{-t} \mper \label{eqn:31}
	\end{align}
	
	For simplicity, let $P = (2-O(\delta))\tau^{1/2}d - 6\hat{\tau}^{1/2} = (2-O(\delta)-o(1))\tau^{1/2}d$ and $Q(\alpha) = \|\alpha_S\|_4^4 - 3\|\alpha_S\|^2$. Then we have that suppose $P > Q(\alpha)$, by taking $t = \frac{(P-Q(\alpha))^2}{36\norm{\alpha_S}^2}$ in equation~\eqref{eqn:31}, 
	\begin{align}
	\Pr\left[A_S \ge P\mid v_k\right]% & =  \Pr\left[A_S - \Exp\left[A_S\right] \ge P-Q\right]\nonumber \\
	%	& = \Pr\left[\sum_{i\in S}\alpha_i^2 (\inner{v_i,\bar{b}_i}^2 - 1) \le -(P-Q)/3\right] \nonumber\\
	& \le \exp\left(-\frac{(P-Q(\alpha))^2}{36\norm{\alpha_S}_4^4}\right)% \tag{by ~\cite[Lemma 1]{laurent2000}}
	\end{align} %Therefore, suppose $\|\alpha_S\|_4^4 - 3\|\alpha_S\|^2 < \tau^{1/2}$
	Hence, we have 
	\begin{align}
	\Pr\left[M'\succeq 0 \wedge E_2''\right]\le \Exp\left[\Pr\left[A_S \ge P\mid v_k\right]\right] \le \left\{\begin{array}{cc}
	\exp\left(-\frac{(P-Q(\alpha))^2}{36\norm{\alpha_S}_4^4}\right) & \textup{if $P > Q(\alpha)$} \\
	1 & \textup{otherwise}
	\end{array}\right.\nonumber
	\end{align}
\end{proof} 
 
For notational convenience, again we define $T_3(\alpha)$ and $T_4(\alpha)$ as,
\begin{align}
T_3(\alpha)  &=\left(\frac{Q(\alpha_S)^2}{\sixmoments{\alpha_S}} \right)^{d/2} \nonumber\\
T_4(\alpha) &=\left(\frac{Q(\alpha_L)^2}{\sixmoments{\alpha_L}} \right)^{d/2}\mper\label{eqn:def_Ts}
\end{align}
Intuitively, $T_3$ and $T_4$ are the contribution of the small coordinates and large coordinates to the quantity $\Exp[\trace(M)]^d p_{g\mid \alpha}(0) \propto Q(\alpha)(\norm{\alpha}_6^6)^{-d/2}$, which is the central object that we are controlling. 

Using Lemma~\ref{lem:prob_indicator}, we show that bounding $\Exp\left[h(\alpha)\indicator{F_k}\right]$ reduces to bounding the second moments of $T_1(\alpha), \dots, T_{4}(\alpha)$. 
\begin{lemma} \label{lem:Ts}
	Let $T_1(\alpha),T_2(\alpha), T_3(\alpha), T_4(\alpha)$ be defined as above. In the setting of Proposition~\ref{prop:f_k}, we have, 
	\begin{align}
	\Exp\left[	h(\alpha)\indicator{F_k}\right] 
& \lesssim \pi^{d/2} (d/(2e))^{-d/2} \max\{\Exp[T_1(\alpha)^2]^{1/2},\Exp\left[T_2(\alpha)^2\right]^{1/2}\}\nonumber\\
& ~~\cdot  \max\left\{\Exp\left[T_3(\alpha)^2\right]^{1/2},\Exp\left[T_4(\alpha)^2\right]^{1/2}, (d/1500)^{d/2}\right\}\mper \nonumber
	\end{align}
\end{lemma}





\begin{proof}[Proof of Lemma~\ref{lem:Ts}] %\Tnote{Clean up the notation, underbrace places}
	By AM-GM inequality (Claim~\ref{claim:amgm}) we obtain that 
	\begin{align}
	\det(M)\indicator{M\succeq 0}& \le (d-1)^{-(d-1)}|\trace(M)|^{d-1}\indicator{M\succeq 0}\mper \label{eqn:50}
	\end{align}
	It follows that, 
	\begin{align}
	W(\alpha)\indicator{F_k} 
	& \le \Exp\left[\frac{|\trace(M)|^{d-1}}{(d-1)^{d-1}}\indicator{M\succeq 0} \indicator{F_k} \mid g = 0, \alpha\right] \indicator{E_0} \tag{by equation~\eqref{eqn:50}} \nonumber \\
	& \le	\underbrace{\Exp\left[\left(\frac{|\trace(M)|}{d-1}\right)^{2(d-1)}\mid g = 0, \alpha\right]^{1/2}}_{:=T_5(\alpha)} \underbrace{\Exp\left[\indicator{M\succeq 0}\indicator{F_k}\mid g = 0, \alpha\right]^{1/2}\indicator{E_0}}_{:=T_6(\alpha)} \label{eqn:46}
	\end{align}
	Here in the last step we used Cauchy-Schwarz inequality. 
	\Tnote{This might be another place that we lose some constant }
%	%Now we will use Proposition~\ref{prop:det-to-trace} to bound the equation above. Let $y  = w =\alpha$ in Proposition~\ref{prop:det-to-trace}. When $E_0$ happens, $\|w\|_{\infty}^2 \le \|w\|_4^2\le \|w\|_{\infty} \|w\| = \|\alpha\|_{\infty} \|\alpha\| \le 2\delta\sqrt{d}\sqrt{n}$. Therefore, $\max\{4p\|w\|_{\infty}^2, 2 \sqrt{pd}\|w\|_4^2\}\le O(\delta) \cdot d^{3/2}n^{1/2}$. Therefore taking $\epsilon = O(\delta)$ in Proposition~\ref{prop:det-to-trace}, we obtain that 
%	\begin{align}
%	\Exp\left[|\trace(M)|^{2(d-1)}\mid g = 0, \alpha\right] \lesssim (1+O(\delta))^{2d} \max\left\{\mu^{2(d-1)}, \left(0.1d^{3/2}n^{1/2}\right)^{2(d-1)}\right\}\label{eqn:61}
%	\end{align}
	%where $\mu = \left|\Exp\left[\trace(M)\right]\right| = (d-1) (\|\alpha\|^4 - 3\|\alpha\|^2 + \frac{3\|\alpha\|_8^8}{\|\alpha\|_6^6})$. 
	Let $T_5(\alpha)$ be defined as in equation~\eqref{eqn:46}, by Corollary~\ref{cor:tracepower}
	\begin{align}
	T_{5}(\alpha)^2\indicator{E_0}\indicator{E_2} \le (1+O(\delta))^{2d} \max\left\{Q(\alpha)^{2d}, (0.1d)^{2d}, \left(0.1pd^{-1/2}n^{1/2}\right)^{2d}\right\}\mper\label{eqn:52}
	\end{align}
	%We observe that when $E_0$ happens, $\mu = (d-1) (\|\alpha\|^4 - 3\|\alpha\|^2 + \frac{3\|\alpha\|_8^8}{\|\alpha\|_6^6})\le (1+O(\delta)) (d-1)\max\{\norm{\alpha}_4^4-3\norm{\alpha}^2, 0.1d\}$. 
	
	
	Then, combining  equation~\eqref{eqn:52} and~\eqref{eqn:41}, we obtain that 
	\begin{align}
	T_5(\alpha)	p_{g\mid \alpha}(0) \indicator{E_0}\indicator{E_2}
	& \le (1+O(\delta))^d (2\pi)^{-d/2} (\Norm{\alpha}_6^6)^{-d/2} \max\left\{Q(\alpha)^d, \left(0.1d^{1/2}n^{1/2}\right)^{d}\right\} \indicator{E_0}\nonumber\\
	& \le (1+O(\delta))^d (\pi)^{-d/2}\max\left\{\left(\frac{Q(\alpha_S)^2}{\sixmoments{\alpha_S}} \right)^{d/2},\left(\frac{Q(\alpha_L)^2}{\sixmoments{\alpha_L}} \right)^{d/2}, \left(d/1500\right)^{d/2}\right\} \indicator{E_0}\label{eqn:57}
	\end{align}
		Here the last inequality uses Cauchy-Schwarz inequality and Holder inequality (technically,  Lemma~\ref{lem:1} with $\eta = 1/2$). \Tnote{Could be tightened by choosing other $\eta$. }
	Using Lemma~\ref{lem:prob_indicator}, we obtain that 
	\begin{align}
	%\Exp\left[\indicator{M\succeq 0}\indicator{F_k}\mid g = 0, \alpha\right]^{1/2}\indicator{E_0}
	T_6(\alpha)
	\le \exp\left(-\frac{(P-Q(\alpha_S))^2}{36\norm{\alpha_S}_4^4}\right)  + \indicator{P \le Q(\alpha_S)}\mper\label{eqn:62}\end{align}
	%where $P = (2-O(\delta))\tau^{1/2}d$.
	
	
 Now we have that our final target can be bounded by 
	\begin{align}
	\Exp\left[	h(\alpha)\indicator{F_k}\right] &= \Exp\left[\Vol(\sphere^{d-1}) W(\alpha) p_{g\mid \alpha}(0)\indicator{F_k}\right] \nonumber\\
	&\lesssim \pi^{d/2} (d/(2e))^{d/2} \Exp\left[ T_6(\alpha)\Fk (T_5(\alpha) p_{g\mid \alpha}(0) \indicator{E_0}\indicator{E_2})\right] \tag{by equation~\eqref{eqn:46}}\\
	& \le  \pi^{d/2} (d/(2e))^{-d/2} \Exp\left[\max\{T_1(\alpha),T_2(\alpha)\}\cdot \max\left\{T_3(\alpha),T_4(\alpha), (d/1500)^{d/2}\right\}\indicator{E_0}\right] \tag{by equation~\eqref{eqn:62} and~\ref{eqn:57}}\\
	& \lesssim \pi^{d/2} (d/(2e))^{-d/2} \max\{\Exp[T_1(\alpha)^2\Ezero]^{1/2},\Exp\left[T_2(\alpha)^2\right]^{1/2}\}\nonumber\\
	& ~~\cdot  \max\left\{\Exp\left[T_3(\alpha)^2\right]^{1/2},\Exp\left[T_4(\alpha)\right]^{1/2}, (d/1500)^{d/2}\right\} \mper \tag{by Cauchy-Schwarz inequality}
	\end{align}
	\end{proof}
	
The next few Lemmas are devoted to controlling the second moments of $T_1(\alpha),\dots, T_{4}(\alpha)$. We start off with $T_{3}(\alpha)$. 
\begin{lemma}\label{lem:moment_small_entries}
In the setting of Lemma~\ref{lem:Ts}, we have, 
	\begin{align}
	\Exp\left[T_3(\alpha)^2\Ezero\right]^{1/2}
	& \le (1+O(\delta))^d \left(\frac{82d}{15e}\right)^{d/2}\mper\nonumber
	\end{align}
\end{lemma}


\begin{proof}
	%Let $C = \max\{C_1,C_2\}$. 
	Let $Z = \Norm{\alpha_S}_4^4 - \Norm{\alpha_S}^2 = \sum_{i=1}^{n} (\alpha_i^4-3\alpha_i^2)\indicator{|\alpha_i| \le \sqrt{C\log d}}$. Then $Z$ is a sub-exponential random variable with parameters $(\sqrt{41n}, 4C\log d)$ (by Lemma~\ref{lem:bernstein_moment}). Moreover, for sufficiently large $C$ (depending on the choice of $\delta$) we have $|\Exp\left[Z\right]|\le \delta$. Therefore, by Lemma~\ref{lem:sub-exp-before_truncation-moments}, choosing $\epsilon = O(\delta)$, we have 
	\begin{align}
	 \Exp\left[Q(\alpha_S)^{2d}\right]=\Exp\left[|Z|^{2d}\right] &\le (1+O(\delta))^{2d}\cdot ((\sqrt{41n})^{2d} (2d)!! + (2C\log d)^{2d} (2d)!) \nonumber\\
	& \le (1+O(\delta))^d(\sqrt{41n})^{2d} (2d)!! \tag{\FIXME{?}Since $\delta n\ge 2d\log d$}\nonumber\\
	& \le (1+O(\delta))^d \left(82nd/e\right)^{d}\nonumber\mper
	\end{align}
	Moreover, when $E_0$ happens, we have $\Norm{\alpha_S}_6^6\ge 15(1-\delta)n$. Hence,
	\begin{align}
	\Exp\left[T_3(\alpha)^2\Ezero\right] = \Exp\left[Q(\alpha_S)^{2d} (\Norm{\alpha_S}_6^6)^{-d}\indicator{E_0}\right] & \le 	(1+O(\delta))^d \left(82nd/e\right)^{d}\cdot  (15(1-\delta)n)^{-d}\nonumber\\
	& \le (1+O(\delta))^d \left(\frac{82d}{15e}\right)^{d}\mper \nonumber
	\end{align}
\end{proof}

Next we control the second moments of $T_4(\alpha)$. 
\begin{lemma}\label{lem:moment_large_entries}
	In the setting of Lemma~\ref{lem:Ts}, we have
	\begin{align}
	\frac{Q(\alpha_L)^2}{\sixmoments{\alpha_L}} \indicator{E_0}\le (1+\delta) d\nonumber\mper
	\end{align}
	As a direct consequence, we have 
	\begin{align}
	\Exp\left[T_4(\alpha)^2\indicator{E_0}\right]^{1/2} \le (1+\delta)^d d^{d/2}\mper\nonumber
	\end{align}
\end{lemma}

\begin{proof}
	We have 
	\begin{align}
	\left(\norm{\alpha_L}^4-3\norm{\alpha_L}^2\right)^2 \indicator{E_0}
	& \le \left(\sum_{i\in L} \alpha_i^6\right)  \left(\sum_{i\in L}(\alpha_i-3/\alpha_i)^2\right) \tag{By Cauchy-Schwarz Inequality}\\
	&\le \Norm{\alpha_L}_6^6\Norm{\alpha_L}^2\indicator{E_0}\tag{since for $i\in L$, $(\alpha_i-3/\alpha_i)^2\le \alpha_i^2$}\\
	& \le \sixmoments{\alpha_L} (1+\delta) d\indicator{E_0}\mper\tag{since when $E_0$ happens, $\norm{\alpha}\le (1+\delta)d$}
	%\tag{by Cauchy-Schwarz}\\
	\end{align}
	%	Hence, we have, 
	%	\begin{align}
	%	\Exp\left[\left(\Norm{\alpha_L}_4^4 - \Norm{\alpha_L}^2 \right)^{d} (\Norm{\alpha_L}_6^6)^{-d/2}\indicator{E_0}\right] &\le  \Exp\left[\Norm{\alpha_L}^d\indicator{E_0}\right] \le (1+\delta)^d d^{d/2}\mper\nonumber 
	%	\end{align}
\end{proof}


The next two Lemmas control the second moments of $T_1(\alpha)$ and $T_2(\alpha)$. 

\begin{lemma}\label{lem:2}
	In the setting of Lemma~\ref{lem:Ts},  we have  
	\begin{align}
	\Exp\left[T_2(\alpha)^2\right] \le (0.1)^d\mper
	\end{align}
\end{lemma}
\begin{proof}
Since  $Q(\alpha_S)$ is a sub-exponential random variable with parameters $(\sqrt{41n}, 4C\log d)$ (by Lemma~\ref{lem:bernstein_moment}), we have that (by Lemma~\ref{lem:sub-exp-property})
\begin{align}
\Pr\left[Q(\alpha)\ge P\right] & \le \exp((2-O(\delta))Kd/82) + \exp(-\sqrt{Knd}/(8C\log d))\nonumber \\
& \lesssim \exp((2-O(\delta))Kd/82) \le (0.01)^d \mper\tag{since $K \ge 2000$ and $n\ge \beta d\log^2 d$ for sufficiently large $\beta$ (that depends on $\delta$)}
\end{align}
\end{proof}

\begin{lemma}\label{lem:3}
	In the setting of Lemma~\ref{lem:Ts},  we have  
	\begin{align}
	\Exp\left[T_1(\alpha)^2\Eone\right] \le (0.1)^d
	\end{align}
	\end{lemma}

\begin{proof}
	Similarly to the proof of Lemma~\ref{lem:2}, we have that for $K \ge 400$, it holds that $\Pr\left[Q(\alpha)\ge P/2\right] \le (0.1)^d$. Then it follows that 
	\begin{align}
	\Exp\left[T_1(\alpha)^2\Ezero\right] & \le \Exp\left[1\mid Q(\alpha)\ge P/2\right]\Pr\left[Q(\alpha)\ge P/2\right]  \nonumber\\
	& + \Exp\left[\exp(-\frac{P^2}{144\fourmoments{\alpha_S}})\Ezero\mid Q(\alpha) < P/2\right]\Pr\left[Q(\alpha)< P/2\right] \nonumber \\
	& \le (0.1)^d + \exp(-Kd/432) \lesssim (0.01)^d\mper  \tag{for $K \ge 2\cdot10^3$.}
	\end{align}
\end{proof}
%
%\begin{corollary}\label{cor:moments_division_bounds}
%	\begin{align}
%	\Exp\left[	\left(\Norm{\alpha}_4^4-\Norm{\alpha}^2\right)^d (\Norm{\alpha}_6^6)^{-d/2}\indicator{E_0}\right]
%	& \le 2^{d/2}(1+O(\delta))^d\left(\frac{41d}{15e}\right)^{d/2}\nonumber
%	\end{align}
%\end{corollary}
%
%\begin{proof}
%	We have, 
%\begin{align}
%	\left(\Norm{\alpha}_4^4-\Norm{\alpha}^2\right)^d (\Norm{\alpha}_6^6)^{-d/2}& \le \left(\frac{2(\Norm{\alpha_S}_4^4 - \Norm{\alpha_S}^2)^2+2 (\Norm{\alpha_L}_4^4 - \Norm{\alpha_L}^2)^2 }{\Norm{\alpha_S}_6^6+\Norm{\alpha_L}_6^6}\right)^{d/2} \nonumber\\
%	& \le 2^{d/2}\left(\max\left\{\frac{(\Norm{\alpha_S}_4^4 - \Norm{\alpha_S}^2)^2}{\Norm{\alpha_S}_6^6}, \frac{(\Norm{\alpha_L}_4^4 - \Norm{\alpha_L}^2)^2}{\Norm{\alpha_L}_6^6}\right\}\right)^{d/2}\nonumber
%\end{align}
%Therefore, taking expectation on both sides, 
%\begin{align}
%\Exp\left[	\left(\Norm{\alpha}_4^4-\Norm{\alpha}^2\right)^d (\Norm{\alpha}_6^6)^{-d/2}\indicator{E_0}\right]& \le 2^{d/2}(1+O(\delta))^d\left\{\left(\frac{41d}{15e}\right)^{d/2}, d^{d/2}\right\} \tag{by Lemma~\ref{lem:moment_small_entries} and Lemma~\ref{lem:moment_large_entries}}\mper \\
%& \le 2^{d/2}(1+O(\delta))^d\left(\frac{41d}{15e}\right)^{d/2}\nonumber
%\end{align}
%\end{proof}


Finally using the four Lemmas above and Lemma~\ref{lem:Ts}, we can prove Proposition~\ref{prop:f_k}. 


\begin{proof}[Proof of Proposition~\ref{prop:f_k}]
	Using Lemma~\ref{lem:Ts}, Lemma~\ref{lem:moment_small_entries},~\ref{lem:moment_large_entries}, \ref{lem:2},\ref{lem:3}, we have that 
	\begin{align}
	\Exp\left[	h(\alpha)\indicator{F_k}\right] 
	& \lesssim \pi^{d/2} (d/(2e))^{d/2} \max\{\Exp[T_1(\alpha)^2]^{1/2},\Exp\left[T_2(\alpha)^2\right]^{1/2}\}\nonumber\\
	& ~~\cdot  \max\left\{\Exp\left[T_3(\alpha)^2\right]^{1/2},\Exp\left[T_4(\alpha)\right]^{1/2}, (d/1500)^{d/2}\right\} \nonumber \\
	& \lesssim \pi^{d/2} (d/(2e))^{-d/2}\cdot\left(\frac{82d}{15e}\right)^{d/2} (0.01)^{d/2}\le (0.3)^d\mper\nonumber\end{align}
\end{proof}


%	\FIXME{TO complete the rest of the proof using Lemma~\ref{lem:2},~\ref{lem:3},\ref{lem:moment_large_entries},\ref{lem:moment_small_entries}}



%
%\begin{corollary}
%	We have that 
%	\begin{align}
%\Exp\left[|\trace(M_S)|^{d-1}\mid g = 0, \alpha\right] \lesssim (1+O(\delta))^{d} d^d\\
%	\Exp\left[|\trace(M_L)|^{d-1}\mid g = 0, \alpha\right] \lesssim (1+O(\delta))^{d} d^d
%	\end{align}
%
%\end{corollary}
%
%\begin{proof}
%	We deal with $|\trace(M_S)|^{d-1} $ and $|\trace(M_L)|^{d-1}$ separately. First we will use Proposition~\ref{prop:det-to-trace} to bound the expectation of $|\trace(M_S)|^{d-1} $. Let $y= \alpha$ and $w\in \R^n$ be such that $w_i = \alpha_i\indicator{\alpha_i^4 < \tau} = \alpha_i\indicator{i\in S}$. Then we have that $(M_S,g)\mid \alpha$ has the same joint distribution as $(M_w,g_y)$ in Proposition~\ref{prop:det-to-trace}. Then we have that 
%	\begin{align}
%	& \Exp\left[|\trace(M_S)|^{d-1}\indicator{M\succeq 0}\indicator{F_k}\mid g = 0, \alpha\right] \indicator{E_0}\\
%	& \le	\Exp\left[|\trace(M_S)|^{d-1}\indicator{F_k}\mid g = 0, \alpha\right]\indicator{E_0}\\
%	&  \le \max\left\{(1+\epsilon)^dd^d	\Exp\left[\trace(M_S)\indicator{F_k}\mid g = 0, \alpha\right]^{d-1} \tag{by Proposition~\eqref{prop:det-to-trace}}
%	, \left(1+\frac{1}{\epsilon}\right)^d\max\left\{4d\|w\|_{\infty}^2, 4d\|w\|_{4}^2\right\}^d\right\} \indicator{E_0}%\tag{\FIXME{using Proposition~\ref{prop:det-to-trace}}}
%	\end{align}
%\end{proof}




==> intro_stripped.tex <==
\begin{abstract}

Tensors decomposition is the key algorithmic tool for learning many latent variable models. 
Many applications require decomposing over-complete tensors with the rank higher than the dimension. Existing provable algorithms for over-complete tensor decomposition often use complicated techniques. However, in practice,   maximizing a simple non-convex objective function $f(\cdot)$ using gradient ascent solves the problem efficiently. 

In this paper we analyze the landscape of the function $f(\cdot)$. We show that if a local maximum has function value that is $(1+\delta)$ factor larger than the expected value of a {\em random point} for any $\delta>0$, then it must be close to one of the components of the tensor. This implies that if one can initialize at a point that is slightly better than the random guess in function value, the gradient ascent algorithm is guaranteed to find one component of the tensor. 


\end{abstract}



\section{Introduction}
\Tnote{Hidden Markov Model  -- $>$ hidden Markov model }

\Tnote{potential points: we don't know where saddle points are }


Tensor decomposition has been widely used as a key algorithmic tool in learning many latent variable models, including Hidden Markov Models, Mixture of Gaussians, topic models and Independent Component Analysis \cite{Chang96,MR06,HKZ12,AHK12,SpectralLDA,HK13-mog}.

In practice,  non-convex optimization based  heuristics such as alternating least squares~\cite{comon2009tensor} and power method~\cite{kolda2011shifted} are popular and empirically successful. However, the theoretical analysis for these algorithms is  limited to either the orthogonal case\cite{RGtensor, ge2015escaping} or local convergence\cite{RGovercomplete1}. This paper aims to understand why these algorithms work in practice by examining the structure of local maxima for the non-convex objective that is commonly used for tensor decomposition.


We focus particularly on the over-complete case of tensor decomposition, meaning the case when the rank $n$ is larger than dimension $d$.  It is particularly useful for learning over-complete representations~\cite{rgDict2, de2007fourth}, where the hidden representations have higher dimension than the data.  For example, in Hidden Markov models, this corresponds to the case when the number of hidden states is larger than the number of possible observations. Previous algorithmic results for this case either requires access to  high order tensors \cite{bhaskara2014smoothed, fourierpca}, or use complicated techniques such as FOOBI or Sum-of-Squares\cite{de2007fourth,ge2015decomposing, MSS16}.



Concretely, we consider decomposing a random 4-th order tensor $T$ of the rank $n$ of the following form, 
$$
T = \sum_{i=1}^n a_i \otimes a_i \otimes a_i \otimes a_i.
$$

Here the vectors $a_i \in \R^d$ are assumed to be drawn i.i.d from Gaussian distribution $N(0, I)$. We call the $a_i$'s the components of the tensor. We are given the entries of tensor $T$ and our goal is to recover the components $a_1,\dots, a_n$. 

We will analyze the following popular non-convex objective, 
\begin{align}
\max & \quad f(x) = \sum_{i,j,k,l\in [d]^4} T_{i,j,k,l} x_ix_jx_kx_l = \sum_{i=1}^n\inner{a_i,x}^4,\label{eq:obj}\\
s.t. & \quad \|x\| = 1.\nonumber
\end{align}


It is known that projected gradient ascent with a proper finite learning rate on objective $f(\cdot)$ is exactly equivalent to the power method, and empirically it finds one of the components $a_i$'s even if $n$ is significantly larger than $d$. 
Moreover, it is proved that around each of $a_i$'s and $-a_i$'s, there is a local maximum, and one of them is the global maximum~\cite{RGovercomplete1}.  However, it remains an major open question whether there is any other spurious local optimum that gradient ascent can potentially converge to. 


\subsection{Main Results}



Our main results rule out the possibility of bad local maxima in a (relatively large) level set. 

\begin{theorem}\label{thm:main_intro} Let $d$ be sufficiently large, and $\epsilon, \delta \in (0,1)$ be two arbitrary constants.   Suppose $d^{1+\epsilon} < n < d^{2-\epsilon}$. Then, with high probability over the randomness of $a_i$'s, we have that  in the superlevel set 
	\begin{align}
	L = \left\{x\in \sphere^{d-1}: f(x) \ge 3(1+\delta)n\right\} \mcom
	\end{align}
	there are exactly $2n$ local maxima with function values $(1\pm o(1))d^2$, each of which is close to one of $a_i$'s or $-a_i$'s, 
	
	\end{theorem}


Note that a random point $z$ on the unit sphere has expected function value $\E[f(z)] = 3n$. Therefore the level set $\mathcal{B}$ contains all points that have function values barely larger than that of the random guess. Thus, Theorem~\ref{thm:main} implies that with a slightly stronger initialization than the random guess, gradient ascent will guarantee to find one of the components in polynomial time. 



\subsection{Related Works}

{\bf Overcomplete tensor decomposition.} Overcomplete tensor decompositions are important in applications such as learning Hidden Markov Models, Independent Component Analysis or Mixture of Gaussians. Many algorithms were proposed for over-complete tensor decomposition. However, some of these algorithms \cite{bhaskara2014smoothed, fourierpca} require higher order tensor than what is required by identifiability results. 
Other algorithms \cite{de2007fourth, ge2015decomposing, MSS16} use complicated techniques such as FOOBI or Sum-of-Squares, and is also not widely used in practice. In practice, the most popular and successful algorithm is the Alternating Least Squares\cite{comon2009tensor} or the power method~\cite{kolda2011shifted}, while theoretically they are only known to converge to optimum with very good initialization. \cite{anandkumar2016analyzing} analyzes the dynamics for power method, while the analysis only requires a reasonably good initialization that is independent with the tensor. 

{\bf Non-convex optimization.} It has been shown that (stochastic) gradient descent~\cite{ge2015escaping,lee2016gradient} or trusted-region algorithms~\cite{sun2015nonconvex} can converge to a local minimum efficiently. Therefore, if all the local minima of the non-convex objective function are global minimum (or the desired solutions), then these algorithms will guarantee to succeed.  Indeed, several non-convex problems have been proved to admit this nice property, including undercomplete tensor decomposition\cite{ge2015escaping}, orthogonal dictionary learning~\cite{sun2015nonconvex}, phase retrieval, synchronization problems~\cite{bandeira2016low}, matrix sensing~\cite{bhojanapalli2016personal} and matrix completion~\cite{ge2016matrix}. 


{\bf Connection to spin-glass model} Before our work, Kac-Rice formula has been applied to counting the number local optima of the spin-glass model in physics, where the main object to study is the landscape of a polynomial with random coefficients. 
Auffinger et al.\cite{auffinger2013random, auffinger2013complexity} give exact formulas for the (expected) number of critical points with any specific index.  The independence between the coefficients allows the use of random matrix theory to characterize the eigenvalue distribution of the Hessian with exact closed-form formula. In comparison, our objective function is a random degree-4 polynomial with a \textit{special} structure and the coefficients therefore are \textit{far} from independent. 
This makes the corresponding random matrix problems much more challenging (see more details in Section~\ref{sec:proof_sketches}).




==> kac-rice-proof_stripped.tex <==


\begin{proof}[Proof of Lemma~\ref{lem:using-kac-rice-zero}]
	The proof follows from equation~\eqref{eqn:102}, the Kac-Rice formula (equation~\eqref{eqn:110}), and law of total expectation (Lemma~\ref{lem:conditioning}). Here we formally justify the use of Kac-Rice formula. We will apply~\cite[Theorem 12.1.1]{adler2009random}. 
	
	First of all, we observe that $f, \nabla f$, $\nabla^2 f$ has continuous density when $n \ge 5$. This is because a sum of $n \ge 5$ powers of (independent or not ) Gaussians has continuous density. Moreover, with probability 1, $f, \nabla f, \nabla^2 f$, as function of $x$, are continuous in the ambient space $\R^d$ and on the unit sphere. We pick an orthonormal frame field $E$ of the manifold $\sphere^{d-1}$.  
	Taking $f^*=\nabla f_E$ in our case, and taking $h^*= (\hessian f, x)$. We will apply ~\cite[Theorem 12.1.1]{adler2009random} with $(f,h)$ there replaced by $(f^*,h*)$. We see these choices satisfy the condition a)-g) in~\cite[Theorem 12.1.1]{adler2009random}. 
	Let $B$ be the interior of the set $\{\textup{PSD matrices}\}\otimes Z$ where $Z = L_1\cap L_2\cap L_G$. 
Thus $B$'s boundary $\partial B$ has finite Hausdorff $(d-1)$-measure. 

	
	We have that  $(\nabla f^*_E)_{ij} = E_{i}f^*_j  = E_iE_jf$, and that $f^*(x) = 0$ if and only if $\grad f(x) = 0$. Therefore, by~\cite[Theorem 12.1.1]{adler2009random}, we obtain, 
	\begin{align}
	\Exp\left[\left|\cM_f\cap L_1\cap L_2\cap L_G\right|\right] &= \Exp\left[|\cM_f \cap Z|\right] \nonumber\\
	 &= \int_{\sphere^{d-1}} \Exp\left[\left|\det(\nabla f^*_E)\right|\indicator{\hessian f\succeq 0}\indicator{x\in Z}\mid f^* = 0\right] p_{f^*}(0) dx\nonumber\\
	&  = \int_{\sphere^{d-1}} \Exp\left[\left|\det(E_iE_j f)\right|\indicator{\hessian f\succeq 0}\indicator{x\in Z}\mid \grad f = 0\right] p_{\grad f}(0) dx \label{eqn:1}
	\end{align}
	Moreover, we recall that the Hessian $\hessian f$ can be also written as $\hessian f = E_iE_j f -  \nabla_{E_i} E_j f$ where here $\nabla_{E_i}$ denotes the Riemannian connection inherited from Euclidean space. Note that conditioned on $\nabla f_E = [E_1f,\dots, E_{d-1}f] = 0$, we have that $\hessian f = E_iE_j f$.  Thus we can replace $E_iE_jf$ by $\hessian f$ in equation~\eqref{eqn:1} and complete the proof. 
	
\end{proof}



==> lowerbound_stripped.tex <==
\section{Lower bounds}

We conjecture the following bound on the number of local optima of $f$. 

\begin{conjecture}
	Suppose $d \ll n \ll n^{1.5}$, then there exists some constant $c > 0$, such that 
	\begin{align}
	\Exp\left[|L|\right] \ge (1+c)^d
	\end{align}
\end{conjecture}

\Tnote{Possible plan for the proof below: }

We will use Lemma~\ref{lem:2}. 
We have 
\begin{align}
	p_{g\mid \alpha}(0) = (2\pi)^{-d/2} (\Norm{\alpha}_6^6)^{-d/2}
\end{align}

and 
\begin{align}
\Vol(\sphere^{d-1}) = \frac{\pi^{(d-1)/2}}{\Gamma(\frac{d+1}{2})}
\end{align}
For simplicity, let 
$$u(\alpha) := \Exp\left[\left|\det(M)\right|\indicator{M\succeq 0} \mid g = 0,\alpha\right] (\Norm{\alpha}_6^6)^{-d/2}$$
We believe that $u(\alpha)$ is large mostly at those $\alpha$ that satisfy \begin{enumerate}
	\item[a)] all of $\alpha_i$'s are not so large, that is, $|\alpha_i| \lesssim 1$. 
	\item[b)] $\norm{\alpha}_4^4 - 3\norm{\alpha}^2 \approx C\sqrt{nd}$ for some constant $C$. 
\end{enumerate}



Note that a) and b) happens with probability at least $C^{-d}$ for some other constant $C$. (Below we will abuse the notation by using  $C$ to denote many different constants. ). We also believe when a) and b) happens, conditioned on $\alpha$,  $M$ is morally independent with $g$ (see Claim~\ref{claim:remove_conditioning} below for some concrete statement). We hope that in this case, 
\begin{align}
3\sum_{i=1}^{n} \alpha_i^2 b_ib_i^{\top}  \approx 3\norm{\alpha}^2 \Id \pm O(\sqrt{nd})\Id
\end{align}
and therefore 
$M = \norm{\alpha}_4^4 \cdot \Id -3\sum_{i=1}^{n} \alpha_i^2 b_ib_i^{\top}  $ is w.h.p a PSD matrix. Then we can lowerbound $\det(M)\indicator{M\succeq 0}$ by 

\begin{align}
\det(M)\ge \left(\norm{\alpha}_4^4 - 3\Norm{\sum_{i=1}^{n} \alpha_i^2 b_ib_i^{\top} }\right)^d \ge \left(C\sqrt{nd}\right)^d
\end{align}
for some constant $C$ (which is different from the previous $C$). 

Finally, a) and b) happens with probability $C^{-d}$ for some constant $C$. Putting these together we obtain that 

\begin{align}
	\Exp\left[|L|\right] & \ge \underbrace{d^{d/2}}_{\Vol(\sphere^{d-1})}\cdot \underbrace{C^d}_{\textup{prob. of a),b)}}\cdot \underbrace{C\sqrt{nd}^d}_{\textup{lower bounds of $\det(M)$}}\cdot \underbrace{(15n)^{-d/2}}_{p_{g\mid \alpha}(0)~\textup{when a) and b) occur}} \\
	& = C^d 
\end{align}
for some $C$. Therefore, the question is that how large this final $C$ will be. We conjecture that it is large than 1. (If it's smaller than 1 then it's even better)



==> macro_stripped.tex <==

\newcommand{\sfrac}[2]{#1\nicefrac{}{#2}}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{question}{Question}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Proposition}
\theoremstyle{definition}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}{Remark}[section]
\numberwithin{equation}{section}
\newcommand{\Os}[1]{= O^*(#1)}
\newcommand{\Oms}[1]{ = \Omega^*(#1)}

\newcommand{\IGNORE}[1]{}

\newcommand{\citep}{\cite}
\newcommand{\citet}{\cite}
\newcommand{\citealp}{\cite}
\def\nn{\nonumber}

\newcommand\E{\mathbb{E}}

\def\Pbb{\mathbb{P}}

\renewcommand\t{{\scriptscriptstyle\top}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\Astar}{\tilde{A}}
\DeclareMathOperator{\Bstar}{\tilde{B}}
\DeclareMathOperator{\Cstar}{\tilde{C}}
\DeclareMathOperator{\wstar}{\tilde{w}}
\DeclareMathOperator{\astar}{\tilde{a}}
\DeclareMathOperator{\bstar}{\tilde{b}}
\DeclareMathOperator{\cstar}{\tilde{c}}
\newcommand\wh{\widehat}
\newcommand\wt{\widetilde}



\newcommand\h{\hat}

\newcommand\tl{\tilde}
\newcommand\inner[1]{\langle #1 \rangle}
\newcommand\sign{\operatorname{sign}}
\newcommand\poly{\operatorname{poly}}
\newcommand\polylog{\operatorname{polylog}}
\newcommand\supp{\operatorname{supp}}
\newcommand\Proj{\operatorname{Proj}}
\newcommand\Diag{\operatorname{Diag}}
\DeclareMathOperator{\range}{range}
\newcommand{\Exp}{\mathop{\mathbb E}\displaylimits}
\newcommand{\tildO}[1]{\tilde{O}(#1)}
\newcommand{\since}[1]{\textrm{Since #1}}
\newcommand{\unitcircle}{\mathcal{K}}


\newcommand{\fourmoments}[1]{\Norm{#1}_4^4}
\newcommand{\sixmoments}[1]{\Norm{#1}_6^6}
\newcommand{\Idx}{P_x}
\newcommand{\sphere}{S}
\newcommand{\inneraix}{\inner{a_i,x}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\tangent}{T}
\newcommand{\Diff}{\nabla}
\newcommand{\indicator}[1]{\mathbf{1}(#1)}
\newcommand{\Vol}{\textup{Vol}}
\newcommand{\bartau}{\bar{\tau}}
\newcommand{\allones}{\mathbf{1}}


\newcommand{\argmax}{\textup{argmax}}
\newcommand{\argmin}{\textup{argmin}}
\newcommand{\mathand}{~~\textup{and}~~}
\newcommand{\set}[1]{{\{#1\}}}
\newcommand{\Set}[1]{{\left\{#1\right\}}}
\newcommand{\hessian}{\textup{Hess }}
\newcommand{\grad}{\textup{grad }}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\Id}{\textup{Id}}


\newcommand{\conj}{^*}
\newcommand{\neighbor}{\mathcal{N}_{\tau}}
\newcommand{\sstar}{s}
\newcommand{\qstar}{q}
\newcommand{\hatG}{\widehat{G}}
\newcommand{\hats}{\hat{s}}
\newcommand{\hatr}{\hat{r}}
\newcommand{\hatq}{\hat{q}}
\newcommand{\thetax}{\theta}
\newcommand{\mper}{\,.}
\newcommand{\mcom}{\,,}

\newcommand{\hatH}{\widehat{H}}
\newcommand{\hatw}{\hat{w}}
\newcommand{\hatp}{\hat{p}}
\newcommand{\hatA}{\hat{A}}
\newcommand{\hatB}{\hat{B}}
\newcommand{\hatC}{\hat{C}}
\newcommand{\hatD}{\hat{D}}
\newcommand{\hath}{\hat{h}}
\newcommand{\haty}{\hat{y}}
\newcommand{\hatv}{\hat{v}}
\newcommand{\hata}{\hat{a}}
\newcommand{\hatc}{\hat{c}}
\newcommand{\hatTheta}{\widehat{\Theta}}
\newcommand{\dy}{\Delta y}
\renewcommand{\dh}{\Delta h}



\newcommand{\dc}{\Delta c}
\newcommand{\da}{\Delta a}
\newcommand{\dA}{\Delta A}
\newcommand{\dq}{\Delta q}
\newcommand{\hatx}{\hat{x}}
\newcommand{\starx}{x^*}
\newcommand{\RHS}{\textup{RHS}}
\newcommand{\of}{\textup{of}}
\newcommand{\CONDNAME}{{weakly-quasi-convex}\xspace}
\newcommand{\CONDADJ}{{weakly-quasi-convex}\xspace}
\newcommand{\CONDNOUN}{{weak quasi convexity}\xspace}
\newcommand{\CONDSHORT}{{WQC}}
\newcommand{\ball}{\mathcal{B}}
\newcommand{\proj}[1]{\Pi_{#1}}
\newcommand{\pnorm}[1]{\|#1\|_p}
\newcommand\R{\mathbb{R}}
\newcommand\C{\mathbb{C}}
\newcommand\N{\mathcal{N}}
\newcommand{\Integer}{\mathbb{Z}}

\newcommand{\ballC}{\mathcal{C}}
\newcommand{\cset}{\mathcal{S}}
\newcommand{\elloneball}{\mathcal{B}}

\newcommand{\finalball}{\mathcal{B}}

\newcommand{\spp}[1]{^{(#1)}}
\newcommand{\hatf}{\hat{f}}

\newcommand{\flambda}{f_{\lambda}}

\newcommand{\glambda}{g_{\lambda}}

\newcommand{\hatflambda}{\hatf_{\lambda}}
\newcommand{\partialgrad}[2]{{\frac{\partial #1 }{\partial #2}}}
\newcommand{\tp}[2]{(#1^{\top})^{#2}}
\newcommand{\OC}{\textup{OC}}
\newcommand{\CC}{\textup{CC}}
\newcommand{\BR}{\textup{BR}}
\newcommand{\MCC}{\textup{MCC}}

\newcommand{\cnorm}{N_C}
\newcommand{\anorm}{Q}

\newcommand{\knorm}[1]{\|#1\|_{\kappa}}



\newcommand{\pbar}{q}
\newcommand{\phat}{q}
\newcommand{\Var}{\textup{Var}}
 
\newcommand{\nin}{\ell}
\newcommand{\nout}{\ell'}
\newcommand{\trace}{\textup{tr}}
\newcommand{\biginner}[1]{\left\langle #1\right \rangle}
\newcommand{\mfA}{\mathfrak{A}}
\newcommand{\hatmfA}{\hat{\mathfrak{A}}}


\newcommand{\Ef}{\bar{f}}
\newcommand{\Rshort}{ER}




\let\epsilon=\varepsilon

\numberwithin{equation}{section}




\newcommand\MYcurrentlabel{xxx}

\newcommand{\MYstore}[2]{	\global\expandafter \def \csname MYMEMORY #1 \endcsname{#2}}

\newcommand{\MYload}[1]{	\csname MYMEMORY #1 \endcsname}

\newcommand{\MYnewlabel}[1]{	\renewcommand\MYcurrentlabel{#1}	\MYoldlabel{#1}}

\newcommand{\MYdummylabel}[1]{}

\newcommand{\torestate}[1]{		\let\MYoldlabel\label	\let\label\MYnewlabel	#1	\MYstore{\MYcurrentlabel}{#1}		\let\label\MYoldlabel}

\newcommand{\restatetheorem}[1]{		\let\MYoldlabel\label
	\let\label\MYdummylabel
	\begin{theorem*}[Restatement of \prettyref{#1}]
		\MYload{#1}
	\end{theorem*}
	\let\label\MYoldlabel
}

\newcommand{\restatelemma}[1]{		\let\MYoldlabel\label
	\let\label\MYdummylabel
	\begin{lemma*}[Restatement of \prettyref{#1}]
		\MYload{#1}
	\end{lemma*}
	\let\label\MYoldlabel
}

\newcommand{\restateprop}[1]{		\let\MYoldlabel\label
	\let\label\MYdummylabel
	\begin{proposition*}[Restatement of \prettyref{#1}]
		\MYload{#1}
	\end{proposition*}
	\let\label\MYoldlabel
}

\newcommand{\restatefact}[1]{		\let\MYoldlabel\label
	\let\label\MYdummylabel
	\begin{fact*}[Restatement of \prettyref{#1}]
		\MYload{#1}
	\end{fact*}
	\let\label\MYoldlabel
}

\newcommand{\restate}[1]{		\let\MYoldlabel\label
	\let\label\MYdummylabel
	\MYload{#1}
	\let\label\MYoldlabel
}


==> setup_stripped.tex <==










==> temp_stripped.tex <==
\begin{proof}
	With slight abuse of notation, we will assume view $\alpha$ as a fixed vector and assumes that it satisfies $F_k$ and $E_0$ throughout the proof, and omit the indicator $\indicator{F_k}$ and $\indicator{E_0}$. 
	
	Let $q = (\alpha_1^3,\dots, \alpha_n^3)^{\top}\in \R^n$, and let $\bar{q} = q/\|q\|$.	Let $z_1,\dots z_{d-1}$ be independent Gaussian random variables in $\R^d$ with covriance $\N(0,\Id_n-\bar{q}\bar{q}^{\top})$. Let $Z$ denote the matrix with $z_i^{\top}$ as rows and let $v_j,j\in [n]$ denotes the columns of $Z$. Then, a$(M\mid g = 0, \alpha)$ has the same distribution as $M'$ defined below \Tnote{To add explanation},
	\begin{align}
	M' = \|\alpha\|_4^4 \Id_{d-1} -3\sum_{i\in [n]} \alpha_i^2v_iv_i^{\top}\mper
	\end{align}
	Moreover, the indicator function $\indicator{E_1}\mid g=0$ has the same distribution as $\indicator{E_1'} = \indicator{\forall i, \|v_i\|^2 \ge (1-\delta)d}$. Then, it suffices to bound from above the quantity 
$$
\Pr\left[M'\succeq 0\wedge E_1'\right]\mper
$$
	A technical complication here is that $v_1,\dots, v_n$ are not independent random variables. We get around this issue by the following ``coupling'' technique which introduces some addition randomness. Let $\beta\in \N(0,\Id_{d-1})$ be a random variable that is independent with the $v_i$'s. Let $\tilde{B} = \beta\bar{q}^{\top}  + Z$. We can verify that $\tilde{B}$ contains independent entries with distribution $\N(0,1)$. Let $\tilde{b}_1,\dots, \tilde{b}_n$ be the columns of $\tilde{B}$. Let $\bar{v}_k = v_k/\norm{v_k}$.  We have that $M'\succeq 0$ implies that 
	\begin{align}
	\bar{v}_k^{\top}M'\bar{v}_k= \|\alpha\|_4^4 - 3\sum_{i\in [n]}\alpha_i^2 \inner{v_i,\bar{v}_i}^2 \ge 0 \label{eqn:23}
	\end{align}
	We divide the coordinates into two subsets: let $S = \{i : \alpha_i^4 \le  \hat{\tau}\}$ and $L = \{i : \alpha_i^4 >\hat{\tau}\}$ where $\hat{\tau}$ satisfies that $\hat{\tau}/\tau \le \epsilon$ for some sufficiently small constant $\epsilon > 0$ and $\hat{\tau} > C\log^2 d$ for a sufficiently large constant $C$.  Let $\alpha_S,\alpha_L\in \R^n$ denote the vectors obtained by zeroing out coordinates of $\alpha$ outside subsets $S$ and $L$ respectively. Note that by definition, when $F_k$ happens we have $k\in L$. We have that when $F_k, E_0$ both happen, 
	
	\begin{align}
	\bar{v}_k^{\top}M'\bar{v}_k & = \norm{\alpha_{S}}_4^4 -3 \sum_{i\in S}\alpha_i^2 \inner{v_i,\bar{v}_i}^2 + \norm{\alpha_L}_4^4 - 3\sum_{i\in L} \alpha_i^2 \inner{v_i,\bar{v}_i}^2 \nonumber\\
	&\le \underbrace{\norm{\alpha_{S}}_4^4 - 3\sum_{i\in S}\alpha_i^2 \inner{v_i,\bar{v}_i}^2}_{A_S} + \underbrace{\norm{\alpha_L}_4^4 - 3\alpha_k^2\inner{v_k,\bar{v}_k}^2}_{A_L} \label{eqn:24}
	\end{align}
	
 		
		Then we have that when $E_0$ happens, $(1+\delta) n\ge \norm{\alpha_L}^2\ge \hat{\tau}^{1/2}|L|$, and it follows that $|L|\le (1+\delta)n/(\Delta\log d)$. Therefore, when $E_0$ happens we have $\norm{\alpha_L}^2 \le (1+\delta)d$. Therefore, $\norm{\alpha_L}_4^4 \le \max_i \alpha_i^2 \cdot \norm{\alpha_L}^2\le (1+\delta)d\max_i \alpha_i^2 = (1+\delta)d\alpha_k^2$. Moreover, when $E_1'$ happens, we have that $\alpha_k^2\inner{v_k,\bar{v}_k}^2 = \alpha_k^2\norm{\bar{v}_k}^2 \ge \alpha_k^2 (1-\delta)d $. Thus, 	\begin{align}
A_L\cdot \indicator{E_1'} &= (\norm{\alpha_L}_4^4 - 3\alpha_k^2\inner{v_k,\bar{v}_k}^2)\indicator{E_1'}  \le (1+\delta)d\alpha_k^2 - 3\alpha_k^2(1-\delta)d \nonumber\\ & \le - (2-O(\delta))\alpha_k^2 d \le -(2-O(\delta))\sqrt{\tau}d\label{eqn:25}
	\end{align}
	Then combining equation~\eqref{eqn:23}, ~\eqref{eqn:24} and~\eqref{eqn:25},  we have that when $M'\succeq 0$ and $E'$ both happen, it holds that $A_S\ge (2-O(d))\tau^{1/2}d$. Next we consider in more detail the random variable $A_S$. Define random variable $Y = \bar{v}_k^{\top} \tilde{B}_{-k}\diag((\alpha_{S})_{-k})$, where $\tilde{B}_{-k}$ is the $(d-1)\times (n-1)$ sub-matrix of $\tilde{B}$ that excludes the $k$-th column of $\tilde{B}$, and $(\alpha_{S})_{-k}$ is the $n-1$-dimensional vector that is obtained from removing the $k$-th entry of $\alpha_S$. Note that since $k\not\in S$, we have that $\norm{Y}^2 = \sum_{i\in S}\alpha_i^2 \inner{v_i,\bar{v}_i}^2$, and $A_S  = \norm{\alpha_S}_4^4 - 3\norm{Y}^2$. Thus our goal next is to understand the distribution of $Y$. 
	
	We observe that $Y\mid v_k$ is a Gaussian random variable since $\tilde{B}_k\mid v_k$ is a Gaussian random variable. Let $\ell_i\in \R^{n-1}$ denote the $i$-th row of the matrix $\tilde{B}$. Then $\ell_1,\dots, \ell_{d-1}$ are i.i.d Gaussian random variable with distribution $\N(0,\Id_{n})$. Now we consider $\ell_i\mid v_{k,i}$, where $v_{k,i}$ is the $i$-th coordinates of vector $v_k$.  Note that $v_{k,i} = z_{i,k} = ((\Id-\bar{q}\bar{q}^{\top})\ell_i)_k = \inner{e_k- \bar{q}_k\bar{q}, \ell_i}$ (here $z_{i,k}$ denotes the $k$-th coordinate of $z_i$ and $e_k$ is the $k$-th natural basis vector in $\R^n$). Thus, conditioning on $v_{k,i}$ imposes linear constraints on $\ell_i$. Let $s_k = e_k- \bar{q}_k\bar{q}\in \R^n$ and $\bar{s}_k  = s_k/\norm{s_k}$. Then $\ell_i \mid v_{k,i}$ has covariance $\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}$. 	 Computing the mean of $\ell_i \mid v_{k,i}$  will be tedious but fortunately our bound will not be sensitive to it. Now we consider random variable  $\ell_i' = (\ell_i)_{-k}\diag((\alpha_{S})_{-k})\mid v_{k,i}$ in $\R^{n-1}$ where $(\ell_i)_{-k}$ denotes the restriction of $\ell_{i}$ to the subset $[n]\backslash \{k\}$. Note that $\ell_i'$ is precisely a row of  $\tilde{B}_{-k}\diag((\alpha_{S})_{-k})$. We have $\ell_i'$ is again a Gaussian random variable and its covariance matrix is $\Sigma = \diag((\alpha_{S})_{-k})\left(\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}\right)_{-k,-k}\diag((\alpha_{S})_{-k})$, where $\left(\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}\right)_{-k,-k}$ is the restriction of $\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}$ to the subsets $([n]\backslash \{k\})\times ([n]\backslash \{k\})$. Since $\ell_i$'s are independent with each other, we have $Y^{\top} \mid \bar{v}_k= [\ell_1',\dots, \ell_{d-1}']\cdot \bar{v}_k$  is Gaussian random variable with covariance $\|\bar{v}_k\|^2\Sigma = \Sigma$. 
	 
	 Next we apply Lemma~\ref{lem:norm_concentration} on random variable $Y^{\top}$ and obtain that $Y^{\top}$ has concentrated norm in the sense that for any choice of $v_k$, 
		\begin{align}
		\Pr\left[\norm{Y}^2 \ge \trace(\Sigma) -\norm{\Sigma} - 2\sqrt{\trace(\Sigma^2)t}\mid v_k\right]\ge 1-e^{-t} \mper\label{eqn:30}
		\end{align}
	 
	 Recall that $\Sigma = \diag((\alpha_{S})_{-k})\left(\Id_{n} - \bar{s}_k\bar{s}_{k}^{\top}\right)_{-k,-k}\diag((\alpha_{S})_{-k})$. Therefore, we have $\trace(\Sigma) = \sum_{i\in S}\alpha_i^2 - \norm{\bar{s}_k\odot (\alpha_S)_{-k}}^2\ge \sum_{i\in S}\alpha_i^2 - \norm{\alpha_S}_{\infty}^2\ge \sum_{i\in S}\alpha_i^2 - \hat{\tau}^{1/2}$. Moreover, we have that $\norm{\Sigma}\le \norm{\alpha_S}^2\le \hat{\tau}^{1/2}$ and $\trace(\Sigma^2)\le \norm{\alpha_S}_4^4$.  Plugging these into equation~\eqref{eqn:30}, and using the fact that $A_S  = \norm{\alpha_S}_4^4 - 3\norm{Y}^2$, we have that for any $t\ge 0$, 
	 \begin{align}
	 \Pr\left[A_S \ge \norm{\alpha_S}_4^4 - 3 \norm{\alpha_S}^2 + 6\hat{\tau}^{1/2} + 6\sqrt{\norm{\alpha_S}^4_4 t}\mid v_k\right]\le e^{-t} \mper \label{eqn:31}
	 \end{align}
	 
	For simplicity, let $P = (2-O(\delta))\tau^{1/2}d - 6\hat{\tau}^{1/2} = (2-O(\delta)-o(1))\tau^{1/2}d$ and $Q(\alpha) = \|\alpha_S\|_4^4 - 3\|\alpha_S\|^2$. Then we have that suppose $P > Q(\alpha)$, by taking $t = \frac{(P-Q(\alpha))^2}{36\norm{\alpha_S}^2}$ in equation~\eqref{eqn:31}, 
	\begin{align}
	 \Pr\left[A_S \ge P\mid v_k\right]\\\\	& \le \exp\left(-\frac{(P-Q(\alpha))^2}{36\norm{\alpha_S}_4^4}\right)	\end{align} 	Hence, we have 
	\begin{align}
	\Pr\left[M'\succeq 0 \wedge E_1'\right]\le \Exp\left[\Pr\left[A_S \ge P\mid v_k\right]\right] \le \left\{\begin{array}{cc}
		\exp\left(-\frac{(P-Q(\alpha))^2}{36\norm{\alpha_S}_4^4}\right) & \textup{if $P > Q(\alpha)$} \\
		1 & \textup{otherwise}
	\end{array}\right.
	\end{align}
\end{proof} 





